Composing Data Stories with Meta Relations

To facilitate the creation of compelling and engaging data stories, AI-powered tools have been introduced to automate the three stages in the workflow: analyzing data, organizing findings, and creating visuals. However, these tools rely on data-level information to derive inflexible relations between findings. Therefore, they often create one-size-fits-all data stories. Differently, our formative study reveals that humans heavily rely on meta relations between these findings from diverse domain knowledge and narrative intent, going beyond datasets, to compose their findings into stylized data stories. Such a gap indicates the importance of introducing meta relations to elevate AI-created stories to a satisfactory level. Though necessary, it is still unclear where and how AI should be involved in working with humans on meta relations. To answer the question, we conducted an exploratory user study with Remex, an AI-powered data storytelling tool that suggests meta relations in the analysis stage and applies meta relations for data story organization. The user study reveals various findings about introducing AI for meta relations into the storytelling workflow, such as the benefit of considering meta relations and their diverse expected usage scenarios. Finally, the paper concludes with lessons and suggestions about applying meta relations to compose data stories to hopefully inspire future research.

==> sections/bio-no-photo.tex <==
\begin{IEEEbiographynophoto}{Haotian Li}
is currently a Ph.D. candidate in Computer Science and Engineering at the Hong Kong University of Science and Technology (HKUST). His main research interests are data visualization, visual analytics, and human-computer interaction. He received his BEng in Computer Engineering from HKUST. For more details, please refer to \url{https://haotian-li.com/}. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Lu Ying} is currently a Ph.D. candidate at the State Key Lab of CAD\&CG, Zhejiang University. Her main research interests are on data storytelling, glyph-based visualization. She is dedicated to integrating the AI technique into visualization to ease the creation of visualization. She received her BEng in Digital Media Technology from Zhejiang University. For more details, please refer to \url{https://yiyinyinguu.github.io/}.
\end{IEEEbiographynophoto}


\begin{IEEEbiographynophoto}{Leixian Shen}
is a PhD student in the Department of Computer Science and Engineering at The Hong Kong University of Science and Technology. He received his master's degree in Software Engineering from Tsinghua University in 2023 and obtained his bachelor's degree in Software Engineering from Nanjing University of Posts and Telecommunications in 2020. His research interests include visual data analysis and storytelling. For more details, please refer to \url{https://shenleixian.github.io/}. 
\end{IEEEbiographynophoto}



\begin{IEEEbiographynophoto}{Yun Wang}
is a senior researcher in the Data, Knowledge, Intelligence (DKI) Area at Microsoft. Her research lies in the intersection of Human-Computer Interaction, and Information Visualization. She develops innovative techniques and interactive systems to facilitate Human-AI Collaboration, Human-Data Interaction, Visual Communication, and Data Storytelling through an interdisciplinary approach. She received her Ph.D. from the Hong Kong University of Science and Technology. For more details, please refer to \url{https://www.microsoft.com/en-us/research/people/wangyun/}. 
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Yingcai Wu} is a Professor at the State Key Lab of CAD\&CG, Zhejiang University.
His main research interests are information visualization and visual analytics, with focuses on urban computing, sports science, immersive visualization, and social media analysis. 
He received his Ph.D. degree in Computer Science from The Hong Kong University of Science and Technology. 
Prior to his current position, Dr. Wu was a postdoctoral researcher in the University of California, Davis from 2010 to 2012, and a researcher in Microsoft Research Asia from 2012 to 2015. 
For more information, please visit \url{http://www.ycwu.org}.
\end{IEEEbiographynophoto}



\begin{IEEEbiographynophoto}{Huamin Qu}
is a chair professor in the Department of Computer Science and Engineering (CSE) at the Hong Kong University of Science and Technology (HKUST) and also the director of the interdisciplinary program office (IPO) of HKUST. He obtained a BS in Mathematics from Xi'an Jiaotong University, China, an MS and a PhD in Computer Science from the Stony Brook University. His main research interests are in visualization and human-computer interaction, with focuses on urban informatics, social network analysis, E-learning, text visualization, and explainable artificial intelligence (XAI). For more information, please visit \url{http://huamin.org/}.
\end{IEEEbiographynophoto}
